PC7 Model: Dynamics of Expanding and Contracting Soft Robots using Piece-wise Constant 7D Deformation Based on Similarity Transformation Group

This paper proposes a novel soft robot model named piece-wise constant 7D deformation (PC7) model that can represent expanding and contracting deformation of, for example, artificial muscle actuator. In the proposed model, we newly define the 7D deformation vector based on SIM(3) - 3D similarity transformation group - whereas a 6D deformation vector was defined for Cosserat rod based on SE(3) - the special Euclid group - in the piece-wise constant strain (PCS) model proposed in the previous study. The additional dimension of the 7D deformation vector represents expanding and contracting deformation, which comes from the scaling parameter in SIM(3). Common mathematical properties between SE(3) and SIM(3) allow us to directly extend the kinematics and dynamics of the PCS model to those of the PC7 model. In particular, we derive the dynamical equation of the PC7 model based on Euler-Poincare equation in a mathematically precise manner. We validate the proposed model through dynamical simulations assuming a thin cylinder structure or McKibben-type artificial muscle actuator.

==> ext_force_mckibben.tex <==
\subsubsection{Generalized External Forces from Kinematic Constraints}
While the kinematic constraints introduced in the previous section strictly restrict the geometric deformation, they alone cannot capture the equilibrium between forces acting in fundamentally different directions. To accurately model the actuator, the mechanical relationship that converts the radial expansion force---induced by the internal pressure---into the axial contraction force must be explicitly defined and incorporated into the model as generalized external forces.

To formulate this, we follow the principle modeled by Chou et al.~\cite{Chou1996}. We consider the virtual work balance between the work $\delta W_{\mathrm{z}}$ done by the equivalent axial contraction force and the work $\delta W_{\mathrm{\alpha}}$ done by the radial expansion. 
Let $\mathcal{F}_{\mathrm{MK},\xi_z}$ denote the axial component of the SIM(3) generalized force. Because the generalized translational force in the PC7 framework is scaled by $\alpha$ relative to the physical force, the actual physical contraction force acting on the length $L$ is represented as $\alpha^{-1}\mathcal{F}_{\mathrm{MK},\xi_z}$. Thus, the equivalence condition $\delta W_{\mathrm{z}} = \delta W_{\mathrm{\alpha}}$ is given by:
\begin{align}
  \delta L \cdot (\alpha^{-1}\mathcal{F}_{\mathrm{MK},\xi_z}) = \delta R \cdot 2\pi P R L.
\end{align}
By substituting the kinematic relationships $R = \alpha R_0$ and $L = \alpha\xi_{lz}$, along with the variational differentials derived from the geometric constraint ($\delta\alpha = \frac{\cos(\phi)}{\sin(\phi_0)} \delta\phi$ and $\delta(\alpha \xi_{lz}) = -\frac{\sin(\phi)}{\cos(\phi_0)} \delta\phi$), the equivalent axial contraction force is obtained as:
\begin{align}
{\mathcal{F}}_{\mathrm{MK,\xi_z}} 
&= -2\pi P R^2_0 \alpha^3 \xi^2_{lz} \tan^{-2}{(\phi_0)}.
\end{align}
As established in the thin-walled cylinder model, the internal fluidic pressure also inherently exerts a direct axial force on the cross-sectional area, yielding the component $\pi P \alpha^3 R_0^2$. Within the spatial derivative framework of the PC7 model, both this direct axial pressure and the mechanically converted contraction force ${\mathcal{F}}_{\mathrm{MK,\xi_z}}$ act simultaneously along the local $z$-axis. Therefore, they are superimposed to construct the total generalized cross-sectional force $\overline{\bm{\mathcal{F}}}_{\mathrm{ext},\xi}$:
\begin{align}
\overline{\bm{\mathcal{F}}}_{\mathrm{ext},\xi} =
\left(\pi P \alpha^3 R_0^2 + {\mathcal{F}}_{\mathrm{MK,\xi_z}}\right)\bm{e}_6 
\end{align}
Crucially, because the inextensible braided sleeve acts as a strict kinematic transmission, the entirety of the radial expansion work is mechanically converted and completely absorbed into the axial cross-sectional force $\overline{\bm{\mathcal{F}}}_{\mathrm{ext},\xi}$. Since no independent radial work is performed outside of this geometric coupling, the distributed radial force density acting on the seventh dimension must be exactly zero ($\bm{\mathcal{F}}_{\mathrm{ext},\alpha} = 0\cdot\bm{e}_7$).
